Velocities of Mesenchymal Cells May be Ill-Defined

The dynamics of single cell migration on flat surfaces is usually modeled by a Langevin-like problem consisting of ballistic motion for short periods and random walk. for long periods. Conversely, recent studies have revealed a previously neglected random motion at very short intervals, what would rule out the possibility of defining the cell instantaneous velocity and a robust measurement procedure. A previous attempt to address this issue considered an anisotropic migration model, which takes into account a polarization orientation along which the velocity is well-defined, and a direction orthogonal to the polarization vector that describes the random walk. Although the numerically and analytically calculated mean square displacement and auto-correlation agree with experimental data for that model, the velocity distribution peaks at zero, which contradicts experimental observations of a constant drift in the polarization direction. Moreover, Potts model simulations indicate that instantaneous velocity cannot be measured for any direction. Here, we consider dynamical equations for cell polarization, which is measurable and introduce a polarization-dependent displacement, circumventing the problem of ill defined instantaneous velocity. Polarization is a well-defined quantity, preserves memory for short intervals, and provides a robust measurement procedure for characterizing cell migration. We consider cell polarization dynamics to follow a modified Langevin equation that yields cell displacement distribution that peaks at positive values, in agreement with experiments and Potts model simulations. Furthermore, displacement autocorrelation functions present two different time scales, improving the agreement between theoretical fits and experiments or simulations.

==> Sections/Abstract.tex <==
\justify{The dynamics of single cell migration on flat surfaces is usually modeled by a Langevin-like problem consisting of ballistic motion for short periods and random walk. 
for long periods. Conversely, recent studies have revealed a previously neglected random motion at very short intervals, what would rule out the possibility of defining the cell instantaneous velocity and a robust measurement procedure. %\cite{Thomas2020,Rita2022}.%Selmeczi, Wu, Dieterich, Li (Journal dependent)., 

A previous attempt to address this issue considered  an anisotropic migration model, which takes into account a polarization orientation along which the velocity is well-defined, and a direction orthogonal to the polarization vector that describes the random walk. Although the numerically and analytically calculated mean square displacement and auto-correlation agree with experimental data for that model, the velocity distribution peaks at zero, which contradicts experimental observations of a constant drift in the polarization direction.
% cite{Nousi2021}
Moreover, Potts model simulations indicate  that instantaneous velocity cannot be measured for any direction. Here, we consider dynamical equations for cell polarization, which is measurable and introduce a polarization-dependent displacement, circumventing the problem of ill defined instantaneous velocity.%\cite{CallanJones2016}. 
Polarization is a well-defined quantity, preserves memory for short intervals, and provides a robust measurement procedure for characterizing cell migration. We consider cell polarization dynamics to follow  a modified Langevin equation that yields cell displacement distribution that peaks at positive values, in agreement with experiments and Potts model simulations. Furthermore, displacement autocorrelation functions present two different time scales, improving the agreement between  theoretical fits and experiments or simulations. 
}



==> bib.tex <==
@article{Graner1992,
   author = {François Graner and James A. Glazier},
   doi = {10.1103/PhysRevLett.69.2013},
   issn = {00319007},
   issue = {13},
   journal = {Physical Review Letters},
   month = {9},
   pages = {2013-2016},
   publisher = {American Physical Society},
   title = {Simulation of biological cell sorting using a two-dimensional extended Potts model},
   volume = {69},
   url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.69.2013},
   year = {1992},
}
@book{CarloBook,
	   title 	= "Introduction to Econophysics: contemporary approaches with Python simulations",
      author 	= "da Cunha, Carlo R.",
      year 	= 2021,
      publisher 	= "CRC Press",
      edition 	= "1$^{\text{st}}$",
      address 	= "Boca Raton, FL"
}
@article{Rens2017,
   author = {Elisabeth G. Rens and Roeland M.H. Merks},
   doi = {10.1016/j.bpj.2016.12.012},
   issn = {15420086},
   issue = {4},
   journal = {Biophysical Journal},
   month = {2},
   pages = {755-766},
   pmid = {28256235},
   publisher = {Biophysical Society},
   title = {Cell Contractility Facilitates Alignment of Cells and Tissues to Static Uniaxial Stretch},
   volume = {112},
   url = {http://dx.doi.org/10.1016/j.bpj.2016.12.012},
   year = {2017},
}
@article{Albert2016,
   author = {Philipp J. Albert and Ulrich S. Schwarz},
   doi = {10.1371/journal.pcbi.1004863},
   editor = {Feilim Mac Gabhann},
   issn = {1553-7358},
   issue = {4},
   journal = {PLOS Computational Biology},
   keywords = {Actins,Adhesives,Cadherins,Cell cycle and cell division,Cell migration,Cell polarity,Ellipses,Surface tension},
   month = {4},
   pages = {e1004863},
   publisher = {Public Library of Science},
   title = {Dynamics of Cell Ensembles on Adhesive Micropatterns: Bridging the Gap between Single Cell Spreading and Collective Cell Migration},
   volume = {12},
   url = {https://dx.plos.org/10.1371/journal.pcbi.1004863},
   year = {2016},
}

@article{Honda1978,
   author = {Hisao Honda},
   doi = {10.1016/0022-5193(78)90315-6},
   issn = {10958541},
   issue = {3},
   journal = {Journal of Theoretical Biology},
   month = {6},
   pages = {523-543},
   pmid = {672241},
   publisher = {Academic Press},
   title = {Description of cellular patterns by Dirichlet domains: The two-dimensional case},
   volume = {72},
   year = {1978},
}


@article{Li2014,
   author = {Bo Li and Sean X. Sun},
   doi = {10.1016/j.bpj.2014.08.006},
   issn = {15420086},
   issue = {7},
   journal = {Biophysical Journal},
   month = {10},
   pages = {1532-1541},
   pmid = {25296305},
   publisher = {Biophysical Society},
   title = {Coherent motions in confluent cell monolayer sheets},
   volume = {107},
   url = {http://dx.doi.org/10.1016/j.bpj.2014.08.006},
   year = {2014},
}

@article{Gardiner2015,
   author = {Bruce S. Gardiner and Kelvin K. L. Wong and Grand R. Joldes and Addison J. Rich and Chin Wee Tan and Antony W. Burgess and David W. Smith},
   doi = {10.1371/journal.pcbi.1004544},
   editor = {Jeffrey J. Saucerman},
   issn = {1553-7358},
   issue = {10},
   journal = {PLOS Computational Biology},
   keywords = {Agent-based modeling,Basement membrane,Buckling,Cell biology,Cell membranes,Cytoplasm,Drag,Extracellular matrix},
   month = {10},
   pages = {e1004544},
   publisher = {Public Library of Science},
   title = {Discrete Element Framework for Modelling Extracellular Matrix, Deformable Cells and Subcellular Components},
   volume = {11},
   url = {https://dx.plos.org/10.1371/journal.pcbi.1004544},
   year = {2015},
}

@article{Niculescu2015,
   author = {Ioana Niculescu and Johannes Textor and Rob J. de Boer},
   doi = {10.1371/journal.pcbi.1004280},
   editor = {Leah Edelstein-Keshet},
   issn = {1553-7358},
   issue = {10},
   journal = {PLOS Computational Biology},
   keywords = {Actins,Cancer cell migration,Cell membranes,Cell migration,Chemokines,Chemotaxis,Simulation and modeling,T cells},
   month = {10},
   pages = {e1004280},
   publisher = {Public Library of Science},
   title = {Crawling and Gliding: A Computational Model for Shape-Driven Cell Migration},
   volume = {11},
   url = {https://dx.plos.org/10.1371/journal.pcbi.1004280},
   year = {2015},
}
@article{Segerer2015,
   author = {Felix J. Segerer and Florian Thüroff and Alicia Piera Alberola and Erwin Frey and Joachim O. Rädler},
   doi = {10.1103/PhysRevLett.114.228102},
   issn = {10797114},
   issue = {22},
   journal = {Physical Review Letters},
   month = {6},
   pages = {228102},
   pmid = {26196648},
   publisher = {American Physical Society},
   title = {Emergence and persistence of collective cell migration on small circular micropatterns},
   volume = {114},
   url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.114.228102},
   year = {2015},
}
@article{vanOers2014,
   author = {René F.M. van Oers and Elisabeth G. Rens and Danielle J. LaValley and Cynthia A. Reinhart-King and Roeland M.H. Merks},
   doi = {10.1371/journal.pcbi.1003774},
   issn = {15537358},
   issue = {8},
   journal = {PLoS Computational Biology},
   keywords = {Cell motility,Endothelial cells,Extracellular matrix,Extracellular matrix adhesions,Finite element analysis,Monte Carlo method,Simulation and modeling,Stiffness},
   month = {8},
   pages = {1003774},
   pmid = {25121971},
   publisher = {Public Library of Science},
   title = {Mechanical Cell-Matrix Feedback Explains Pairwise and Collective Endothelial Cell Behavior In Vitro},
   volume = {10},
   url = {www.ploscompbiol.org},
   year = {2014},
}
@article{Szabo2013,
   author = {András Szabó and Roeland M.H. Merks},
   doi = {10.3389/fonc.2013.00087},
   issn = {2234943X},
   journal = {Frontiers in Oncology},
   keywords = {Cell-based modeling,Cellular potts model,Evolutionary tumor model,Multiscale modeling,Tumor growth model,Tumor invasion model,Tumor metastasis model},
   month = {4},
   pages = {87},
   publisher = {Frontiers},
   title = {Cellular Potts modeling of tumor growth, tumor invasion, and tumor evolution},
   volume = {3 APR},
   url = {www.frontiersin.org},
   year = {2013},
}
@article{Kabla2012,
   author = {Alexandre J. Kabla},
   doi = {10.1098/rsif.2012.0448},
   issn = {1742-5689},
   issue = {77},
   journal = {Journal of The Royal Society Interface},
   keywords = {Active matter,Cell invasion,Collective migration,Epithelium,Wound healing},
   month = {12},
   pages = {3268-3278},
   publisher = {Royal Society},
   title = {Collective cell migration: leadership, invasion and segregation},
   volume = {9},
   url = {https://royalsocietypublishing.org/doi/10.1098/rsif.2012.0448},
   year = {2012},
}
@article{Lober2015,
   author = {Jakob Löber and Falko Ziebert and Igor S. Aranson},
   doi = {10.1038/srep09172},
   issn = {20452322},
   issue = {1},
   journal = {Scientific Reports},
   keywords = {Biomaterials,Computational biophysics,cells},
   month = {3},
   pages = {1-7},
   pmid = {25779619},
   publisher = {Nature Publishing Group},
   title = {Collisions of deformable cells lead to collective migration},
   volume = {5},
   url = {www.nature.com/scientificreports},
   year = {2015},
}
@article{Camley-Rappel2014,
   author = {Brian A. Camley and Wouter Jan Rappel},
   doi = {10.1103/PhysRevE.89.062705},
   issn = {15502376},
   issue = {6},
   journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
   month = {6},
   pages = {062705},
   pmid = {25019812},
   publisher = {American Physical Society},
   title = {Velocity alignment leads to high persistence in confined cells},
   volume = {89},
   url = {https://journals.aps.org/pre/abstract/10.1103/PhysRevE.89.062705},
   year = {2014},
}
@article{Camley2014,
   author = {Brian A. Camley and Yunsong Zhang and Yanxiang Zhao and Bo Li and Eshel Ben-Jacob and Herbert Levine and Wouter Jan Rappel},
   doi = {10.1073/pnas.1414498111},
   issn = {10916490},
   issue = {41},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   month = {10},
   pages = {14770-14775},
   pmid = {25258412},
   publisher = {National Academy of Sciences},
   title = {Polarity mechanisms such as contact inhibition of locomotion regulate persistent rotational motion of mammalian cells on micropatterns},
   volume = {111},
   url = {www.pnas.org/cgi/doi/10.1073/pnas.1414498111},
   year = {2014},
}
@article{Shao2012,
   author = {Danying Shao and Herbert Levine and Wouter Jan Rappel},
   doi = {10.1073/pnas.1203252109},
   issn = {00278424},
   issue = {18},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   keywords = {Actin dynamics,Cell adhesion,Keratocyte,Phase field},
   month = {5},
   pages = {6851-6856},
   pmid = {22493219},
   publisher = {National Academy of Sciences},
   title = {Coupling actin flow, adhesion, and morphology in a computational cell motility model},
   volume = {109},
   url = {https://www.pnas.org/content/109/18/6851 https://www.pnas.org/content/109/18/6851.abstract},
   year = {2012},
}
@article{Ziebert2012,
   author = {Falko Ziebert and Sumanth Swaminathan and Igor S. Aranson},
   doi = {10.1098/rsif.2011.0433},
   issn = {1742-5689},
   issue = {70},
   journal = {Journal of The Royal Society Interface},
   keywords = {Actin self-assembly,Cell motility,Nonlinear physics},
   month = {5},
   pages = {1084-1092},
   publisher = {Royal Society},
   title = {Model for self-polarization and motility of keratocyte fragments},
   volume = {9},
   url = {https://royalsocietypublishing.org/doi/10.1098/rsif.2011.0433},
   year = {2012},
}
@article{Shao2010,
   author = {Danying Shao and Wouter Jan Rappel and Herbert Levine},
   doi = {10.1103/PhysRevLett.105.108104},
   issn = {00319007},
   issue = {10},
   journal = {Physical Review Letters},
   month = {9},
   pages = {108104},
   pmid = {20867552},
   publisher = {American Physical Society},
   title = {Computational model for cell morphodynamics},
   volume = {105},
   url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.105.108104},
   year = {2010},
}
@article{Tarle2017,
   author = {Victoria Tarle and Estelle Gauquelin and S. R.K. Vedula and Joseph D'Alessandro and C. T. Lim and Benoit Ladoux and Nir S. Gov},
   doi = {10.1088/1478-3975/aa6591},
   issn = {14783975},
   issue = {3},
   journal = {Physical Biology},
   keywords = {collective cell migration,curvature-force feedback,leader cells},
   month = {5},
   pages = {035001},
   pmid = {28467320},
   publisher = {Institute of Physics Publishing},
   title = {Modeling collective cell migration in geometric confinement},
   volume = {14},
   url = {https://iopscience.iop.org/article/10.1088/1478-3975/aa6591 https://iopscience.iop.org/article/10.1088/1478-3975/aa6591/meta},
   year = {2017},
}
@article{Alt2017,
   author = {Silvanus Alt and Poulami Ganguly and Guillaume Salbreux},
   doi = {10.1098/rstb.2015.0520},
   issn = {0962-8436},
   issue = {1720},
   journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
   keywords = {Epithelial mechanics,Morphogenesis,Simulations,Tissue mechanics,Vertex models},
   month = {5},
   pages = {20150520},
   publisher = {Royal Society Publishing},
   title = {Vertex models: from cell mechanics to tissue morphogenesis},
   volume = {372},
   url = {https://royalsocietypublishing.org/doi/10.1098/rstb.2015.0520},
   year = {2017},
}
@article{Banerjee2015,
   author = {Shiladitya Banerjee and Kazage J.C. Utuje and M. Cristina Marchetti},
   doi = {10.1103/PhysRevLett.114.228101},
   issn = {10797114},
   issue = {22},
   journal = {Physical Review Letters},
   month = {6},
   pages = {228101},
   publisher = {American Physical Society},
   title = {Propagating Stress Waves during Epithelial Expansion},
   volume = {114},
   url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.114.228101},
   year = {2015},
}
@article{Basan2013,
   author = {Markus Basan and Jens Elgeti and Edouard Hannezo and Wouter Jan Rappel and Herbert Levine},
   doi = {10.1073/pnas.1219937110},
   issn = {00278424},
   issue = {7},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   month = {2},
   pages = {2452-2459},
   pmid = {23345440},
   publisher = {National Academy of Sciences},
   title = {Alignment of cellular motility forces with tissue flow as a mechanism for efficient wound healing},
   volume = {110},
   url = {www.pnas.org/cgi/doi/10.1073/pnas.1219937110},
   year = {2013},
}
@article{Szabo2010,
   author = {A. Szabó and R. Ünnep and E. Méhes and W. O. Twal and W. S. Argraves and Y. Cao and A. Czirók},
   doi = {10.1088/1478-3975/7/4/046007},
   issn = {14783975},
   issue = {4},
   journal = {Physical Biology},
   month = {11},
   pages = {046007},
   pmid = {21076204},
   publisher = {Institute of Physics Publishing},
   title = {Collective cell motion in endothelial monolayers},
   volume = {7},
   url = {https://iopscience.iop.org/article/10.1088/1478-3975/7/4/046007 https://iopscience.iop.org/article/10.1088/1478-3975/7/4/046007/meta},
   year = {2010},
}
@article{Sepulveda2013,
   author = {Néstor Sepúlveda and Laurence Petitjean and Olivier Cochet and Erwan Grasland-Mongrain and Pascal Silberzan and Vincent Hakim},
   doi = {10.1371/journal.pcbi.1002944},
   issn = {1553734X},
   issue = {3},
   journal = {PLoS Computational Biology},
   keywords = {Approximation methods,Autocorrelation,Cell cycle and cell division,Epithelium,Motion,Simulation and modeling,Velocity,Wound healing},
   pages = {1002944},
   pmid = {23505356},
   publisher = {Public Library of Science},
   title = {Collective Cell Motion in an Epithelial Sheet Can Be Quantitatively Described by a Stochastic Interacting Particle Model},
   volume = {9},
   url = {www.ploscompbiol.org},
   year = {2013},
}
@article{Szabo2006,
   author = {B. Szabó and G. J. Szöllösi and B. Gönci and Zs Jurányi and D. Selmeczi and Tamás Vicsek},
   doi = {10.1103/PhysRevE.74.061908},
   issn = {15393755},
   issue = {6},
   journal = {Physical Review E - Statistical, Nonlinear, and Soft Matter Physics},
   month = {12},
   pages = {061908},
   publisher = {American Physical Society},
   title = {Phase transition in the collective migration of tissue cells: Experiment and model},
   volume = {74},
   url = {https://journals.aps.org/pre/abstract/10.1103/PhysRevE.74.061908},
   year = {2006},
}
@article{Goychuk2018,
   author = {Andriy Goychuk and David B. Brückner and Andrew W. Holle and Joachim P. Spatz and Chase P. Broedersz and Erwin Frey},
   journal = {arXiv},
   month = {8},
   publisher = {arXiv},
   title = {Morphology and Motility of Cells on Soft Substrates},
   url = {http://arxiv.org/abs/1808.00314},
   year = {2018},
}
@article{Dietrich2018,
   author = {Miriam Dietrich and Hugo Le Roy and David B. Brückner and Hanna Engelke and Roman Zantl and Joachim O. Rädler and Chase P. Broedersz},
   doi = {10.1039/c8sm00018b},
   issn = {17446848},
   issue = {15},
   journal = {Soft Matter},
   month = {4},
   pages = {2816-2826},
   pmid = {29595213},
   publisher = {Royal Society of Chemistry},
   title = {Guiding 3D cell migration in deformed synthetic hydrogel microstructures},
   volume = {14},
   url = {https://pubs.rsc.org/en/content/articlehtml/2018/sm/c8sm00018b https://pubs.rsc.org/en/content/articlelanding/2018/sm/c8sm00018b},
   year = {2018},
}
@article{Dieterich2008,
   author = {Peter Dieterich and Rainer Klages and Roland Preuss and Albrecht Schwab},
   doi = {10.1073/pnas.0707603105},
   issn = {00278424},
   issue = {2},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   keywords = {Data analysis,Fractional dynamics,Non-Brownian motion},
   month = {1},
   pages = {459-463},
   pmid = {18182493},
   publisher = {National Academy of Sciences},
   title = {Anomalous dynamics of cell migration},
   volume = {105},
   url = {www.pnas.orgcgidoi10.1073pnas.0707603105},
   year = {2008},
}
@article{Albert2014,
   author = {Philipp J. Albert and Ulrich S. Schwarz},
   doi = {10.1016/j.bpj.2014.04.036},
   issn = {15420086},
   issue = {11},
   journal = {Biophysical Journal},
   month = {6},
   pages = {2340-2352},
   pmid = {24896113},
   publisher = {Biophysical Society},
   title = {Dynamics of cell shape and forces on micropatterned substrates predicted by a cellular Potts model},
   volume = {106},
   url = {http://dx.doi.org/10.1016/j.bpj.2014.04.036},
   year = {2014},
}
@article{Camley2013,
   author = {Brian A. Camley and Yanxiang Zhao and Bo Li and Herbert Levine and Wouter Jan Rappel},
   doi = {10.1103/PhysRevLett.111.158102},
   issn = {00319007},
   issue = {15},
   journal = {Physical Review Letters},
   month = {10},
   pages = {158102},
   pmid = {24160631},
   publisher = {American Physical Society},
   title = {Periodic migration in a physical model of cells on micropatterns},
   volume = {111},
   url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.111.158102},
   year = {2013},
}
@article{Ziebert2013,
   author = {Falko Ziebert and Igor S. Aranson},
   doi = {10.1371/journal.pone.0064511},
   issn = {19326203},
   issue = {5},
   journal = {PLoS ONE},
   keywords = {Actin motors,Actin polymerization,Actins,Adhesives,Cell motility,Deformation,Motion,Stiffness},
   month = {5},
   pages = {64511},
   pmid = {23741334},
   publisher = {Public Library of Science},
   title = {Effects of Adhesion Dynamics and Substrate Compliance on the Shape and Motility of Crawling Cells},
   volume = {8},
   url = {www.plosone.org},
   year = {2013},
}

@article{Maree2012,
   author = {Athanasius F.M. Marée and Verônica A. Grieneisen and Leah Edelstein-Keshet},
   doi = {10.1371/journal.pcbi.1002402},
   issn = {1553734X},
   issue = {3},
   journal = {PLoS Computational Biology},
   keywords = {Actin filaments,Actins,Cell membranes,Cell motility,Chemical dynamics,Cytoskeleton,GTPase signaling,Guanosine triphosphatase},
   month = {3},
   pages = {e1002402},
   pmid = {22396633},
   publisher = {Public Library of Science},
   title = {How cells integrate complex stimuli: The effect of feedback from phosphoinositides and cell shape on cell polarization and motility},
   volume = {8},
   url = {http://royalsociety.org/grants/schemes/dorothy-hodgkin/},
   year = {2012},
}
@article{Maree2006,
   author = {Athanasius F.M. Marée and Alexandra Jilkine and Adriana Dawes and Verônica A. Grieneisen and Leah Edelstein-Keshet},
   doi = {10.1007/s11538-006-9131-7},
   issn = {00928240},
   issue = {5},
   journal = {Bulletin of Mathematical Biology},
   keywords = {2D cell motility model,Actin cytoskeleton,Cdc42 Rac Rho,Cellular Potts Model,Chemotaxis,Mathematical model,Small G-proteins},
   month = {7},
   pages = {1169-1211},
   pmid = {16794915},
   publisher = {Springer},
   title = {Polarization and movement of keratocytes: A multiscale modelling approach},
   volume = {68},
   url = {http://theory.bio.uu.nl/stan/keratocyte.},
   year = {2006},
}
@article{Mogilner2009,
   author = {Alex Mogilner},
   doi = {10.1007/s00285-008-0182-2},
   issn = {03036812},
   issue = {1-2},
   journal = {Journal of Mathematical Biology},
   keywords = {Actin,Adhesion,Cell mechanics,Cell motility,Contraction,Protrusion},
   month = {1},
   pages = {105-134},
   pmid = {18461331},
   publisher = {Springer},
   title = {Mathematics of cell motility: Have we got its number?},
   volume = {58},
   url = {https://link.springer.com/article/10.1007/s00285-008-0182-2},
   year = {2009},
}

@article{Wu2014,
   author = {Pei Hsun Wu and Anjil Giri and Sean X. Sun and Denis Wirtz},
   doi = {10.1073/pnas.1318967111},
   issn = {10916490},
   issue = {11},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   keywords = {3D motility,Cancer,Theory},
   month = {3},
   pages = {3949-3954},
   pmid = {24594603},
   publisher = {National Academy of Sciences},
   title = {Three-dimensional cell migration does not follow a random walk},
   volume = {111},
   url = {https://www.pnas.org/content/111/11/3949 https://www.pnas.org/content/111/11/3949.abstract},
   year = {2014},
}

@article{Thüroff2019,
   author = {Florian Thüroff and Andriy Goychuk and Matthias Reiter and Erwin Frey},
   doi = {10.7554/eLife.46842},
   issn = {2050084X},
   journal = {eLife},
   month = {12},
   pmid = {31808744},
   publisher = {eLife Sciences Publications Ltd},
   title = {Bridging the gap between single-cell migration and collective dynamics},
   volume = {8},
   year = {2019},
}
@report{Turing1952,
   author = {A M Turing},
   issue = {641},
   journal = {Philosophical Transactions of the Royal Society of London. Series B, Biological Sciences},
   pages = {37-72},
   title = {The Chemical Basis of Morphogenesis},
   volume = {237},
   url = {http://www.jstor.org/about/terms.html.},
   year = {1952},
}
@article{Potdar2009,
   author = {Alka A. Potdar and Jenny Lu and Junhwan Jeon and Alissa M. Weaver and Peter T. Cummings},
   doi = {10.1007/s10439-008-9592-y},
   issn = {00906964},
   issue = {1},
   journal = {Annals of Biomedical Engineering},
   keywords = {Bimodal framework,Mammalian cell,Random motility coefficient,Turn angle distribution},
   month = {1},
   pages = {230-245},
   pmid = {18982450},
   publisher = {Springer},
   title = {Bimodal analysis of mammary epithelial cell migration in two dimensions},
   volume = {37},
   url = {https://link.springer.com/article/10.1007/s10439-008-9592-y},
   year = {2009},
}
@article{Friedl2011,
   author = {Peter Friedl and Stephanie Alexander},
   doi = {10.1016/j.cell.2011.11.016},
   issn = {00928674},
   issue = {5},
   journal = {Cell},
   month = {11},
   pages = {992-1009},
   pmid = {22118458},
   publisher = {Elsevier},
   title = {Cancer invasion and the microenvironment: Plasticity and reciprocity},
   volume = {147},
   url = {http://www.cell.com/article/S0092867411013547/fulltext http://www.cell.com/article/S0092867411013547/abstract https://www.cell.com/cell/abstract/S0092-8674(11)01354-7},
   year = {2011},
}
@article{Wolf2007,
   author = {Katarina Wolf and Yi I. Wu and Yueying Liu and Jörg Geiger and Eric Tam and Christopher Overall and M. Sharon Stack and Peter Friedl},
   doi = {10.1038/ncb1616},
   issn = {14657392},
   issue = {8},
   journal = {Nature Cell Biology},
   keywords = {Cancer Research,Cell Biology,Developmental Biology,Life Sciences,Stem Cells,general},
   month = {7},
   pages = {893-904},
   pmid = {17618273},
   publisher = {Nature Publishing Group},
   title = {Multi-step pericellular proteolysis controls the transition from individual to collective cancer cell invasion},
   volume = {9},
   url = {https://www.nature.com/articles/ncb1616},
   year = {2007},
}
@article{Qi2018,
   author = {Kai Qi and Na Li and Zhenyu Zhang and Gerry Melino},
   doi = {10.1016/j.cellimm.2017.11.010},
   issn = {10902163},
   journal = {Cellular Immunology},
   keywords = {Immune responses,Mesenchymal stem cells},
   month = {4},
   pages = {86-93},
   pmid = {29221689},
   publisher = {Academic Press Inc.},
   title = {Tissue regeneration: The crosstalk between mesenchymal stem cells and immune response},
   volume = {326},
   year = {2018},
}
@article{Cui2020,
   author = {Biling Cui and Chenchen Zhang and Bin Gan and Wenen Liu and Jiaqiang Liang and Zhiqiang Fan and Yuying Wen and Yang Yang and Xinsheng Peng and Yanfang Zhou},
   doi = {10.1016/j.msec.2019.110611},
   issn = {18730191},
   journal = {Materials Science and Engineering C},
   keywords = {Bone mesenchymal stem cells,Collagen,Scaffold,Skin wound healing,Tussah silk fibroin},
   month = {4},
   pages = {110611},
   pmid = {32228999},
   publisher = {Elsevier Ltd},
   title = {Collagen-tussah silk fibroin hybrid scaffolds loaded with bone mesenchymal stem cells promote skin wound repair in rats},
   volume = {109},
   year = {2020},
}
@article{Fortuna2020,
   author = {Ismael Fortuna and Gabriel C. Perrone and Monique S. Krug and Eduarda Susin and Julio M. Belmonte and Gilberto L. Thomas and James A. Glazier and Rita M.C. de Almeida},
   doi = {10.1016/j.bpj.2020.04.024},
   issn = {15420086},
   issue = {11},
   journal = {Biophysical Journal},
   month = {6},
   pages = {2801-2815},
   pmid = {32407685},
   publisher = {Biophysical Society},
   title = {CompuCell3D Simulations Reproduce Mesenchymal Cell Migration on Flat Substrates},
   volume = {118},
   year = {2020},
}
@article{Rita2022,
   author = {Rita M.C. {de Almeida} and Guilherme S.Y. Giardini and Mendeli Vainstein and James A. Glazier and Gilberto L. Thomas},
   doi = {10.1016/j.physa.2021.126526},
   issn = {03784371},
   journal = {Physica A: Statistical Mechanics and its Applications},
   month = {2},
   pages = {126526},
   publisher = {Elsevier BV},
   title = {Exact solution for the Anisotropic Ornstein–Uhlenbeck process},
   volume = {587},
   year = {2022},
}
@article{Thomas2020,
   author = {Gilberto L. Thomas and Ismael Fortuna and Gabriel C. Perrone and James A. Glazier and Julio M. Belmonte and Rita M.C. de Almeida},
   doi = {10.1016/j.physa.2020.124493},
   issn = {03784371},
   journal = {Physica A: Statistical Mechanics and its Applications},
   keywords = {Cell migration,Fürth equation},
   month = {7},
   pages = {124493},
   publisher = {Elsevier B.V.},
   title = {Parameterizing cell movement when the instantaneous cell migration velocity is ill-defined},
   volume = {550},
   year = {2020},
}
@article{Vicsek1995,
   author = {Tams Vicsek and Andrs Czirk and Eshel Ben-Jacob and Inon Cohen and Ofer Shochet},
   doi = {10.1103/PhysRevLett.75.1226},
   issn = {00319007},
   issue = {6},
   journal = {Physical Review Letters},
   month = {8},
   pages = {1226-1229},
   pmid = {10060237},
   publisher = {American Physical Society},
   title = {Novel type of phase transition in a system of self-driven particles},
   volume = {75},
   url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.75.1226},
   year = {1995},
}
@article{Ross1909,
   author = {H. C. Ross},
   doi = {10.1016/S0140-6736(00)65950-0},
   issn = {01406736},
   issue = {4455},
   journal = {The Lancet},
   month = {1},
   pages = {152-154},
   publisher = {Elsevier},
   title = {ON A COMBINATION OF SUBSTANCES WHICH EXCITES AMŒBOID MOVEMENT IN LEUCOCYTES, BY WHICH LIVING CAN BE DIFFERENTIATED FROM DEAD CELLS.},
   volume = {173},
   year = {1909},
}
@article{WHC,
   author = {W.H.C.},
   doi = {10.1016/s0002-9394(28)92870-6},
   issn = {00029394},
   issue = {10},
   journal = {American Journal of Ophthalmology},
   month = {10},
   pages = {825},
   publisher = {Elsevier BV},
   title = {Ciliary Movement},
   volume = {11},
   url = {http://www.ajo.com/article/S0002939428928706/fulltext}, 
   year = {1928},
}
@article{Furth,
   author = {Reinhold Fürth},
   doi = {10.1007/BF01328731},
   issn = {14346001},
   issue = {3},
   journal = {Zeitschrift für Physik},
   month = {6},
   pages = {244-256},
   publisher = {Springer-Verlag},
   title = {Die Brownsche Bewegung bei Berücksichtigung einer Persistenz der Bewegungsrichtung. Mit Anwendungen auf die Bewegung lebender Infusorien},
   volume = {2},
   year = {1920},
}

@article{Peruani2007,
   author = {Fernando Peruani and Luis G. Morelli},
   doi = {10.1103/PhysRevLett.99.010602},
   issn = {00319007},
   issue = {1},
   journal = {Physical Review Letters},
   month = {7},
   pages = {010602},
   publisher = {American Physical Society},
   title = {Self-propelled particles with fluctuating speed and direction of motion in two dimensions},
   volume = {99},
   url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.99.010602},
   year = {2007},
}

@article{Palsson2000,
   author = {Eirikur Palsson and Hans G. Othmer},
   doi = {10.1073/pnas.97.19.10448},
   issn = {00278424},
   issue = {19},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   month = {9},
   pages = {10448-10453},
   pmid = {10984537},
   publisher = {National Academy of Sciences},
   title = {A model for individual and collective cell movement in Dictyostelium discoideum},
   volume = {97},
   url = {/pmc/articles/PMC27044/?report=abstract https://www.ncbi.nlm.nih.gov/pmc/articles/PMC27044/},
   year = {2000},
}

@article{Hennig2020,
   author = {K. Hennig and I. Wang and P. Moreau and L. Valon and S. DeBeco and M. Coppey and Y. A. Miroshnikova and C. Albiges-Rizo and C. Favard and R. Voituriez and M. Balland},
   doi = {10.1126/sciadv.aau5670},
   issn = {23752548},
   issue = {1},
   journal = {Science Advances},
   month = {1},
   pmid = {31921998},
   publisher = {American Association for the Advancement of Science},
   title = {Stick-slip dynamics of cell adhesion triggers spontaneous symmetry breaking and directional migration of mesenchymal cells on one-dimensional lines},
   volume = {6},
   year = {2020},
}

@article{Camley2017,
   author = {B. A. Camley and W. J. Rappel},
   doi = {10.1088/1361-6463/aa56fe},
   issn = {13616463},
   issue = {11},
   journal = {Journal of Physics D: Applied Physics},
   keywords = {collective migration,modeling,motility},
   month = {2},
   pages = {113002},
   publisher = {Institute of Physics Publishing},
   title = {Physical models of collective cell motility: From cell to tissue},
   volume = {50},
   url = {https://iopscience.iop.org/article/10.1088/1361-6463/aa56fe https://iopscience.iop.org/article/10.1088/1361-6463/aa56fe/meta},
   year = {2017},
}

@article{Lammermann2009,
   author = {Tim Lämmermann and Michael Sixt},
   doi = {10.1016/j.ceb.2009.05.003},
   issn = {09550674},
   issue = {5},
   journal = {Current Opinion in Cell Biology},
   month = {10},
   pages = {636-644},
   pmid = {19523798},
   publisher = {Elsevier Current Trends},
   title = {Mechanical modes of 'amoeboid' cell migration},
   volume = {21},
   year = {2009},
}

@article{Mogilner2020,
   author = {Alex Mogilner and Erin L. Barnhart and Kinneret Keren},
   doi = {10.1016/j.semcdb.2019.10.019},
   issn = {10963634},
   journal = {Seminars in Cell and Developmental Biology},
   keywords = {Actin,Cell mechanics,Cell motility,Fish keratocyte,Lamellipodium,Myosin},
   month = {4},
   pages = {143-151},
   pmid = {31718950},
   publisher = {Elsevier Ltd},
   title = {Experiment, theory, and the keratocyte: An ode to a simple model for cell motility},
   volume = {100},
   year = {2020},
}

@article{Hall2000,
   author = {Alan Hall and Catherine D. Nobes},
   doi = {10.1098/rstb.2000.0632},
   issn = {09628436},
   issue = {1399},
   journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
   keywords = {Actin,GTPase,Migration,Rho},
   month = {7},
   pages = {965-970},
   pmid = {11128990},
   publisher = {Royal Society},
   title = {Rho GTPases: Molecular switches that control the organization and dynamics of the actin cytoskeleton},
   volume = {355},
   url = {https://royalsocietypublishing.org/doi/abs/10.1098/rstb.2000.0632},
   year = {2000},
}

@article{Hall1998,
   author = {Alan Hall},
   doi = {10.1126/science.279.5350.509},
   issn = {00368075},
   issue = {5350},
   journal = {Science},
   month = {1},
   pages = {509-514},
   pmid = {9438836},
   publisher = {American Association for the Advancement of Science},
   title = {Rho GTpases and the actin cytoskeleton},
   volume = {279},
   url = {https://science.sciencemag.org/content/279/5350/509 https://science.sciencemag.org/content/279/5350/509.abstract},
   year = {1998},
}

@article{Kholodenko2006,
   author = {Boris N. Kholodenko},
   doi = {10.1038/nrm1838},
   issn = {14710072},
   issue = {3},
   journal = {Nature Reviews Molecular Cell Biology},
   keywords = {Biochemistry,Cancer Research,Cell Biology,Developmental Biology,Life Sciences,Stem Cells,general},
   month = {3},
   pages = {165-176},
   pmid = {16482094},
   publisher = {Nature Publishing Group},
   title = {Cell-signalling dynamics in time and space},
   volume = {7},
   url = {www.nature.com/reviews/molcellbio},
   year = {2006},
}

@article{Merchant2018,
   author = {Brian Merchant and Leah Edelstein-Keshet and James J. Feng},
   doi = {10.1016/j.ydbio.2018.01.013},
   issn = {1095564X},
   journal = {Developmental Biology},
   keywords = {Cell mechanics,Co-attraction,Contact inhibition of locomotion,Persistence of polarity,Rac1,RhoA,Symmetry-breaking},
   month = {12},
   pages = {S262-S273},
   pmid = {29366821},
   publisher = {Elsevier Inc.},
   title = {A Rho-GTPase based model explains spontaneous collective migration of neural crest cell clusters},
   volume = {444},
   year = {2018},
}

@article{Stossel1990,
 author = {Thomas P. Stossel},
 doi = {10.2307/29774178},
 issn = {00030996},
 journal = {American Scientist},
 number = {5},
 pages = {408--423},
 publisher = {Sigma Xi, The Scientific Research Society},
 title = {How Cells Crawl},
 volume = {78},
 URL = {http://www.jstor.org/stable/29774178},
 year = {1990}
}

@article{Bugyi2020,
   author = {Beáta Bugyi and Miklós Kellermayer},
   doi = {10.1007/s10974-019-09515-z},
   issn = {15732657},
   issue = {1},
   journal = {Journal of Muscle Research and Cell Motility},
   keywords = {Actin,Actomyosin,Albert Szent-Györgyi,Brúnó F. Straub,Ilona Banga,Muscle contraction},
   month = {3},
   pages = {3-9},
   pmid = {31093826},
   publisher = {Springer},
   title = {The discovery of actin: “to see what everyone else has seen, and to think what nobody has thought”*},
   volume = {41},
   url = {https://doi.org/10.1007/s10974-019-09515-z},
   year = {2020},
}

@article{Gail1970,
   author = {Mitchell H. Gail and Charles W. Boone},
   doi = {10.1016/S0006-3495(70)86347-0},
   issn = {00063495},
   issue = {10},
   journal = {Biophysical Journal},
   month = {10},
   pages = {980-993},
   pmid = {5531614},
   publisher = {Cell Press},
   title = {The Locomotion of Mouse Fibroblasts in Tissue Culture},
   volume = {10},
   year = {1970},
}

@article{Selmeczi2005,
   author = {David Selmeczi and Stephan Mosler and Peter H. Hagedorn and Niels B. Larsen and Henrik Flyvbjerg},
   doi = {10.1529/biophysj.105.061150},
   issn = {00063495},
   issue = {2},
   journal = {Biophysical Journal},
   month = {8},
   pages = {912-931},
   pmid = {15951372},
   publisher = {Biophysical Society},
   title = {Cell motility as persistent random motion: Theories from experiments},
   volume = {89},
   year = {2005},
}

@article{Genthon2020,
   author = {Arthur Genthon},
   doi = {10.1140/epjh/e2020-10009-8},
   issue = {1},
   journal = {European Physical Journal H},
   month = {6},
   pages = {49-105},
   publisher = {Springer},
   title = {The concept of velocity in the history of Brownian motion -- From physics to mathematics and vice versa},
   volume = {45},
   url = {http://arxiv.org/abs/2006.05399 http://dx.doi.org/10.1140/epjh/e2020-10009-8},
   year = {2020},
}

@article{Maiuri2015,
   author = {Paolo Maiuri and Jean François Rupprecht and Stefan Wieser and Verena Ruprecht and Olivier Bénichou and Nicolas Carpi and Mathieu Coppey and Simon De Beco and Nir Gov and Carl Philipp Heisenberg and Carolina Lage Crespo and Franziska Lautenschlaeger and Maël Le Berre and Ana Maria Lennon-Dumenil and Matthew Raab and Hawa Racine Thiam and Matthieu Piel and Michael Sixt and Raphaël Voituriez},
   doi = {10.1016/j.cell.2015.01.056},
   issn = {10974172},
   issue = {2},
   journal = {Cell},
   month = {4},
   pages = {374-386},
   pmid = {25799384},
   publisher = {Cell Press},
   title = {Actin flows mediate a universal coupling between cell speed and cell persistence},
   volume = {161},
   url = {https://pubmed.ncbi.nlm.nih.gov/25799384/},
   year = {2015},
}

@article{CallanJones2016,
   author = {Andrew C. Callan-Jones and Raphaël Voituriez},
   doi = {10.1016/j.ceb.2016.01.003},
   issn = {18790410},
   journal = {Current Opinion in Cell Biology},
   keywords = {Actins / metabolism*,Andrew C Callan-Jones,Cell Movement*,Cell Polarity*,MEDLINE,Myosins / metabolism,NCBI,NIH,NLM,National Center for Biotechnology Information,National Institutes of Health,National Library of Medicine,Non-U.S. Gov't,PubMed Abstract,Raphaël Voituriez,Research Support,Review,doi:10.1016/j.ceb.2016.01.003,pmid:26827283},
   month = {2},
   pages = {12-17},
   pmid = {26827283},
   publisher = {Elsevier Ltd},
   title = {Actin flows in cell migration: From locomotion and polarity to trajectories},
   volume = {38},
   url = {https://pubmed.ncbi.nlm.nih.gov/26827283/},
   year = {2016},
}

@article{Giardini2022,
   author = {Guilherme S Y Giardini and Porto Alegre},
   keywords = {Anisotropy,Biophysics,Cell Migration,Polarization,Masters Dissertation},
   title = {A Proper Velocity Measure for Mesenchymal Cells Migration},
   url = {https://lume.ufrgs.br/handle/10183/240303},
   year = {2022},
}

@article{Lemons1997,
   author = {Don S. Lemons and Anthony Gythiel},
   doi = {10.1119/1.18725},
   issn = {0002-9505},
   issue = {11},
   journal = {American Journal of Physics},
   keywords = {01.30,01.65,05.40,Brownian motion,teaching},
   month = {11},
   pages = {1079-1081},
   publisher = {American Association of Physics Teachers (AAPT)},
   title = { Paul Langevin’s 1908 paper “On the Theory of Brownian Motion” [“Sur la théorie du mouvement brownien,” C. R. Acad. Sci. (Paris) 146 , 530–533 (1908)] },
   volume = {65},
   url = {http://aapt.scitation.org/doi/10.1119/1.18725},
   year = {1997},
}

@article{Masuzzo2017,
   author = {Paola Masuzzo and Lynn Huyck and Aleksandra Simiczyjew and Christophe Ampe and Lennart Martens and Marleen Van Troys},
   doi = {10.1038/srep42383},
   issn = {20452322},
   journal = {Scientific Reports},
   month = {2},
   pmid = {28205527},
   publisher = {Nature Publishing Group},
   title = {An end-to-end software solution for the analysis of high-throughput single-cell migration data},
   volume = {7},
   year = {2017},
}

@article{Nousi2021,
   author = {Aimilia Nousi and Maria Tangen Søgaard and Mélanie Audoin and Liselotte Jauffred},
   doi = {10.1016/j.bbrep.2021.101120},
   issn = {24055808},
   journal = {Biochemistry and Biophysics Reports},
   keywords = {Diffusion models,Glioblastoma,Invasion assay,Single-cell tracking},
   month = {12},
   pages = {101120},
   publisher = {Elsevier B.V.},
   title = {Single-cell tracking reveals super-spreading brain cancer cells with high persistence},
   volume = {28},
   year = {2021},
}

@article{Allen2020,
   author = {Greg M. Allen and Kun Chun Lee and Erin L. Barnhart and Mark A. Tsuchida and Cyrus A. Wilson and Edgar Gutierrez and Alexander Groisman and Julie A. Theriot and Alex Mogilner},
   doi = {10.1016/j.cels.2020.08.008},
   issn = {24054720},
   issue = {3},
   journal = {Cell Systems},
   keywords = {actin,adhesion,asymmetry,cell migration,cell motility,cell turning,keratocyte,myosin,self-organization},
   month = {9},
   pages = {286-299.e4},
   pmid = {32916096},
   publisher = {Cell Press},
   title = {Cell Mechanics at the Rear Act to Steer the Direction of Cell Migration},
   volume = {11},
   url = {http://www.cell.com/article/S2405471220302921/fulltext http://www.cell.com/article/S2405471220302921/abstract https://www.cell.com/cell-systems/abstract/S2405-4712(20)30292-1},
   year = {2020},
}

@article{Thomas2022,
   author = {Gilberto L. Thomas and Ismael Fortuna and Gabriel C. Perrone and François Graner and Rita M.C. de Almeida},
   doi = {10.1016/J.PHYSA.2021.126511},
   issn = {0378-4371},
   journal = {Physica A: Statistical Mechanics and its Applications},
   keywords = {Cell polarization,CompuCell3D,Modified Fürth equation,Single-cell migration},
   month = {2},
   pages = {126511},
   publisher = {North-Holland},
   title = {Shape–velocity correlation defines polarization in migrating cell simulations},
   volume = {587},
   year = {2022},
}

@article{Metzner2015,
   author = {Claus Metzner and Christoph Mark and Julian Steinwachs and Lena Lautscham and Franz Stadler and Ben Fabry},
   doi = {10.1038/NCOMMS8516},
   issn = {20411723},
   journal = {Nature Communications},
   month = {6},
   pmid = {26108639},
   publisher = {Nature Publishing Group},
   title = {Superstatistical analysis and modelling of heterogeneous random walks},
   volume = {6},
   year = {2015},
}

@article{Gruver2010,
   author = {J. Scott Gruver and Alka A. Potdar and Junhwan Jeon and Jiqing Sai and Bridget Anderson and Donna Webb and Ann Richmond and Vito Quaranta and Peter T. Cummings and Chang Y. Chung},
   doi = {10.1016/J.BPJ.2010.03.073},
   issn = {15420086},
   issue = {2},
   journal = {Biophysical Journal},
   month = {7},
   pages = {367-376},
   pmid = {20643054},
   publisher = {Biophysical Society},
   title = {Bimodal Analysis Reveals a General Scaling Law Governing Nondirected and Chemotactic Cell Motility},
   volume = {99},
   year = {2010},
}

@article{Jiang2005,
   doi = {10.1073/PNAS.0408954102/SUPPL_FILE/08954FIG13.PDF},
   issn = {00278424},
   issue = {4},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   keywords = {Motility,Polarity,Self-assembled monolayers},
   month = {1},
   pages = {975-978},
   pmid = {15653772},
   publisher = {National Academy of Sciences},
   title = {Directing cell migration with asymmetric micropatterns},
   volume = {102},
   url = {https://www.pnas.org/doi/abs/10.1073/pnas.0408954102},
   year = {2005},
}

@article{Marquadt1963,
 ISSN = {03684245},
 URL = {http://www.jstor.org/stable/2098941},
 author = {Donald W. Marquardt},
 journal = {Journal of the Society for Industrial and Applied Mathematics},
 number = {2},
 pages = {431--441},
 publisher = {Society for Industrial and Applied Mathematics},
 title = {An Algorithm for Least-Squares Estimation of Nonlinear Parameters},
 urldate = {2023-10-31},
 volume = {11},
 year = {1963}
}

@article{Levenberg1944,
   author = {Kenneth Levenberg},
   doi = {10.1090/QAM/10666},
   issn = {0033-569X},
   issue = {2},
   journal = {Quarterly of Applied Mathematics},
   pages = {164-168},
   publisher = {American Mathematical Society (AMS)},
   title = {A method for the solution of certain non-linear problems in least squares},
   volume = {2},
   year = {1944},
}

@article{Martin2021,
   author = {David Martin and Jérémy O'Byrne and Michael E. Cates and Étienne Fodor and Cesare Nardini and Julien Tailleur and Frédéric Van Wijland},
   doi = {10.1103/PHYSREVE.103.032607/FIGURES/7/MEDIUM},
   issn = {24700053},
   issue = {3},
   journal = {Physical Review E},
   month = {3},
   pages = {032607},
   pmid = {33862678},
   publisher = {American Physical Society},
   title = {Statistical mechanics of active Ornstein-Uhlenbeck particles},
   volume = {103},
   url = {https://journals.aps.org/pre/abstract/10.1103/PhysRevE.103.032607},
   year = {2021},
}

@article{Fodor2021,
   author = {Étienne Fodor and Robert L. Jack and Michael E. Cates},
   doi = {10.1146/annurev-conmatphys-031720-032419},
   journal = {Annual Review of Condensed Matter Physics},
   keywords = {dissipation,entropy production,large deviations,nonequilibrium field theories,phase transitions,self-propelled particles},
   month = {4},
   pages = {215-238},
   publisher = {Annual Reviews Inc.},
   title = {Irreversibility and biased ensembles in active matter: Insights from stochastic thermodynamics},
   volume = {13},
   url = {http://arxiv.org/abs/2104.06634 http://dx.doi.org/10.1146/annurev-conmatphys-031720-032419},
   year = {2021},
}

